Deterministic Automata for Unordered Trees

Automata for unordered unranked trees are relevant for defining schemas and queries for data trees in Json or Xml format. While the existing notions are well-investigated concerning expressiveness, they all lack a proper notion of determinism, which makes it difficult to distinguish subclasses of automata for which problems such as inclusion, equivalence, and minimization can be solved efficiently. In this paper, we propose and investigate different notions of "horizontal determinism", starting from automata for unranked trees in which the horizontal evaluation is performed by finite state automata. We show that a restriction to confluent horizontal evaluation leads to polynomial-time emptiness and universality, but still suffers from coNP-completeness of the emptiness of binary intersections. Finally, efficient algorithms can be obtained by imposing an order of horizontal evaluation globally for all automata in the class. Depending on the choice of the order, we obtain different classes of automata, each of which has the same expressiveness as CMso.

==> Makefile <==
top:
	pdflatex 0
	bibtex 0

# shortcuts

s  : short
l  : long
sc : shortComments
lc : longComments
s+ : short+
l+ : long+

# short and long, with and without comments

shortComments:
	pdflatex -synctex=1 "\def\CMPused{}\def\CMPshortC{}\input{0}"
	
longComments:
	pdflatex -synctex=1 "\def\CMPused{}\def\CMPlongC{}\input{0}"
	
short:
	pdflatex -synctex=1 "\def\CMPused{}\def\CMPshort{}\input{0}"
	
long:
	pdflatex -synctex=1 "\def\CMPused{}\def\CMPlong{}\input{0}"

# full compilations; no comments

short+: short 
	bibtex 0
	pdflatex "\def\CMPused{}\def\CMPshort{}\input{0}"
	pdflatex -synctex=1 "\def\CMPused{}\def\CMPshort{}\input{0}"
	cp 0.pdf 00short.pdf

long+: long
	bibtex 0
	pdflatex "\def\CMPused{}\def\CMPlong{}\input{0}"
	pdflatex -synctex=1 "\def\CMPused{}\def\CMPlong{}\input{0}"
	cp 0.pdf 00long.pdf
	
final: short+ long+
	pdflatex appendix-transition
	pdftk 00short.pdf appendix-transition.pdf 00long.pdf cat output 00short-and-long.pdf

	

==> comments.tex <==

\newcommand{\comments}[2]{\quad\\\fbox{\parbox{\linewidth}{{\sc #1}:\\#2}}}
\newcommand{\adrien}[1]{\comments{Adrien}{#1}}
\newcommand{\cedric}[1]{\comments{Cedric}{#1}}
\newcommand{\joachim}[1]{\qquad\\ {\color{green!50!black}{\fbox{\parbox{\linewidth}{{\scshape Joachim}:\\#1}}}\qquad\\}}
\newcommand{\jn}[1]{{\color{green!50!black}{%\marginpar{\bfseries\color{purple!80!black} Joachim}
#1}\color{black}}}
\newcommand{\Joachim}[2]{{\color{green!50!black}{\marginpar{\bfseries\color{green!50!black} Joachim #1}#2}\color{black}}}
\newcommand{\Adrien}[2]{{\color{blue!80!black}{\marginpar{\bfseries\color{blue!80!black} Adrien #1}#2}\color{black}}}
\newcommand{\adrieninline}[1]{{\color{blue!80!black}{\marginpar{\bfseries\color{blue!80!black} Adrien}#1}\color{black}}}
\newcommand{\aurelieninline}[1]{{\color{red!65!black}{\marginpar{\bfseries\color{red!65!black} Aurélien}#1}\color{black}}}
\newcommand{\ralf}[1]{\marginpar{\small Ralf: #1}}

\newcommand{\COMMENT}[2]{\quad\\\fbox{\parbox{\linewidth}{{\sc #2}:\\#1}}}
%\newcommand{\COMMENT}[2]{}

\newcommand{\aurelien}[1]{\comment{#1}{Aurelien}}
\newcommand{\sebastian}[1]{\COMMENT{#1}{Sebastian}}


\newcommand\Gray[1]{{\color{gray}{#1}}}
%\newcommand\Blue[1]{{\color{blue}{#1}}}
%\newcommand\Red[1]{{\color{red}{#1}}}
\newcommand\Green[1]{{\color{green!60!black}{#1}}}

\newcommand{\vh}[2]{{\color{purple!80!black}{\marginpar{\bfseries\color{purple!80!black} Vincent: #1}#2}\color{black}}}
\newcommand{\vhi}[1]{{\color{purple!80!black}{\marginpar{\bfseries\color{purple!80!black} Vincent}#1}\color{black}}}
\newcommand{\VH}[1]{{\color{purple!80!black}{\comments{Vincent}{#1}}}}
\newcommand{\RT}[1]{{\color{green!80!black}{\comments{Ralf}{#1}}}}


==> eptcsdata.tex <==
\providecommand{\firstpage}{189}
\providecommand{\publicationstatus}{Adriano Peron and Carla Piazza (Eds.):\\
Proceedings of the Fifth International Symposium on\\
Games, Automata, Logics and Formal Verification (GandALF 2014)\\
EPTCS 161, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.161.17}{10.4204/EPTCS.161.17}}
\pdfoutput=1


==> mdframedthm.tex <==

\usepackage{starfont} % nice symbols
\usepackage[framemethod=tikz]{mdframed}
\mdfsetup{skipabove=\topskip,skipbelow=0\topskip}

% abbrev, full name, 
\newcommand\getmdfstyle[3]{%
\mdfdefinestyle{#1style}{%
  linecolor=#1color!70!phdback,middlelinewidth=1.0pt,%
  frametitlerule=true,%
  frametitleaboveskip=2.5pt,%
  frametitlebelowskip=1pt,%
  roundcorner=3pt,
  frametitlefont=\bfseries\sffamily\color{#1color}#3\quad,%
  apptotikzsetting={\tikzset{mdfframetitlebackground/.append style={%
                      shade,left color=#1color!10!phdback, right color=#1color!20!phdback}}},
  frametitlerulecolor=#1color!30!phdback,
  frametitlerulewidth=1pt,
  innertopmargin=6pt,
  backgroundcolor=#1color!5!phdback,
}
\mdtheorem[style=#1style]{#1}[thmcounter]{#2}
}

\colorlet{lemcolor}{base02}
\newcounter{thmcounter} \numberwithin{thmcounter}{chapter}
\getmdfstyle{defn}{Definition}{\Water}
\getmdfstyle{thm}{Theorem}{\Air}
\getmdfstyle{lem}{Lemma}{\Earth}
\getmdfstyle{prp}{Proposition}{\Fire} \colorlet{prpcolor}{thmcolor}
\getmdfstyle{cor}{Corollary}{\Air}
\getmdfstyle{cnj}{Conjecture}{\Aquarius}
\getmdfstyle{fcnj}{False Conjecture}{\Neptune}
\getmdfstyle{rem}{Remark}{\Earth}

\mdfdefinestyle{proofstyle}{
  linecolor=base0,
  innertopmargin=0pt,
  backgroundcolor=phdback,
  topline=false,bottomline=false,
  middlelinewidth=1pt,
}

\surroundwithmdframed[style=proofstyle]{proof}
 
\newcommand*\closedbox{%
  \color{base0}\leavevmode\hbox to.77778em{\hfil\rule{.675em}{.675em}\hfil}}
\let\qedsymbol\closedbox

\mdfdefinestyle{examplestyle}{
  linecolor=defncolor!20!phdback,
  innertopmargin=0pt,
  roundcorner=3pt,
  innertopmargin=5pt,
  backgroundcolor=defncolor!7!phdback,
  middlelinewidth=1pt,
}

\nc\eggsymbol{\textbf{\color{base02}$\diamondsuit$}}
\nc\egghere{\hfill\smash\eggsymbol}
\rc\egg[2][1]{\begin{mdframed}[style=examplestyle]%
{\noi\textbf{\textsf{Example:}\ \ }{{#2}}%
\ifnum #1=1 \egghere \fi}
\end{mdframed}}

\mdfdefinestyle{equationhstyle}{
  linecolor=thmcolor!20!phdback,
  roundcorner=3pt,
  innertopmargin=-5.5pt,
  backgroundcolor=thmcolor!7!phdback,
  middlelinewidth=1pt,
}

\surroundwithmdframed[style=equationhstyle]{equationh}


==> no-comments.tex <==

\newcommand{\comments}[2]{}
\newcommand{\adrien}[1]{\comments{Adrien}{#1}}
\newcommand{\cedric}[1]{\comments{Cedric}{#1}}
\newcommand{\joachim}[1]{}
\newcommand{\jn}[1]{#1}
\newcommand{\Joachim}[2]{#2}
\newcommand{\Adrien}[2]{#2}
\newcommand{\adrieninline}[1]{#1}
\newcommand{\ralf}[1]{}

\newcommand{\COMMENT}[2]{}

%\newcommand{\COMMENT}[2]{}



\newcommand\Gray[1]{{\color{gray}{#1}}}
%\newcommand\Blue[1]{{\color{blue}{#1}}}
%\newcommand\Red[1]{{\color{red}{#1}}}
\newcommand\Green[1]{{\color{green!60!black}{#1}}}


\newcommand{\vh}[2]{#2}
\newcommand{\vhi}[1]{}
\newcommand{\VH}[1]{}
\newcommand{\RT}[1]{}

